On Nested Sequents for Constructive Modal Logics

We present deductive systems for various modal logics that can be obtained from the constructive variant of the normal modal logic CK by adding combinations of the axioms d, t, b, 4, and 5. This includes the constructive variants of the standard modal logics K4, S4, and S5. We use for our presentation the formalism of nested sequents and give a syntactic proof of cut elimination.

==> constructive-macros.tex <==
\mathchardef\mhyphen="2D 
\newcommand{\sqCircL}{\ensuremath{[\!\!\mhyphen}} 
\newcommand{\sqCircR}{\ensuremath{]\!\!\mhyphen}}
\newcommand{\lollipop}{\ensuremath{-\!\circ}}  
\newcommand{\CatExam}{\ensuremath{\code{CatExam}\uparrow}} 
\newcommand{\icollapse}{\ensuremath{\code{ICollapse}\!\downarrow}}
\newcommand{\IL}{\code{IL}}
\newcommand{\abot}{\ensuremath{\mathbb{1}}} 
\newcommand{\mtop}{\ensuremath{^*\top}} 
\newcommand{\HBBI}{\code{HBBI}}  
\newcommand{\NCK}{\code{NCK}}
\newcommand{\formulasize}{\ensuremath{\code{f}\_\code{size}}}
\newcommand{\lockfocusAnt}[3]{\ensuremath{\langle}{#1} {\rangle} 
{\parallel}~ {\langle} {#2} {\rangle}~ {\mid}~ {#3}} 
\newcommand{\lockfocus}[4]{\ensuremath{{\langle} {#1} {\rangle} 
{\parallel}~ {\langle} \heavyS{#2} {\rangle}~ {\mid}~ {\heavyS{#3}} \vdash \heavyS{#4}}}
%\newcommand{\hide}[1]{}  
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
\node[shape=circle,draw,inner sep=1pt] (char) {\ensuremath{#1}};}}
\newcommand{\Heap}{\code{Heap}}
\newcommand{\heavyS}{\mathbf}
\newcommand{\apply}{\text{\textbf{apply}}}    
\newcommand{\lift}{\code{lift}}
\newcommand{\LBBI}{\code{LBBI}} 
\newcommand{\length}{\code{len}}
\newcommand{\scenario}{\text{\textbf{scenario}}} 
\newcommand{\posPrincipal}{\code{posPrincipal}}
\newcommand{\pickO}{\text{\textbf{pick1}}}  
\newcommand{\Sc}{\code{Sc}}  
\newcommand{\bolt}{{\normalsize \text{\Lightning}}}
\newcommand{\derivationdepth}{\ensuremath{\code{der}\_\code{depth}}}
\newcommand{\BranchStack}{\code{BranchStack}} 
\newcommand{\BTrackStack}{\code{BTrackStack}}
\newcommand{\pickT}{\text{\textbf{pick2}}}  
\newcommand{\peek}{\code{peek}}
\newcommand{\Node}{\code{Node}} 
\newcommand{\Nd}{\code{Nd}}  
\definecolor{lightsteelblue}{RGB}{176,196,222}
\newcommand{\Phase}{\code{Phase}} 
\newcommand{\PBISq}{\code{PBISq}} 
\newcommand{\ant}{\code{ant}} 
\newcommand{\fillHole}{\code{FillHole}} 
\newcommand{\toBunch}{\code{ToBunch}} 
\newcommand{\toFormula}{\code{ToFormula}} 
\newcommand{\remove}{\code{remove}}
\newcommand{\Mark}{\code{Mark}} 
\newcommand{\cons}{\code{cons}}
\newcommand{\Inf}{\code{Inf}}
\newcommand{\BPS}{\text{\textbf{Backward-Proof-Search}}} 
\newcommand{\Backtrack}{\text{\textbf{Backtrack}}} 
\newcommand{\Finishing}{\text{\textbf{Finishing}}} 
\newcommand{\code}[1]{{\ensuremath{\tt #1}}} 
\newcommand{\NR}{\code{NR}}
\newcommand{\R}{\code{R}}   
\newcommand{\occur}{\code{occur}}
\newcommand{\proj}{\code{proj}}  
\newcommand{\collapse}{\code{collapse}} 
\newcommand{\observe}{\code{observe}}
\newcommand{\Ph}{\code{P}} 
\newcommand{\Rec}{\code{Rec}}  
\newcommand{\process}{\text{\textbf{construct}}}   
\newcommand{\processLock}{\text{\textbf{processLock}}}
\newcommand{\GenScenario}{\text{\textbf{genScenario}}} 
\newcommand{\PosMarker}{\code{PosMark}}
\newcommand{\ScenarioList}{\code{ScenarioList}}
\newcommand{\ScList}{\code{ScList}} 
\newcommand{\MultiCut}{\code{MultiCut}}
\newcommand{\Cut}{\code{Cut}} 
\newcommand{\persist}{\code{persist}}
\newcommand{\OutInt}{\code{out\_int}}
\newcommand{\plusplus}{\text{\textbf{++}}} 
\newcommand{\fetch}{\text{\textbf{fetchSc}}} 
\newcommand{\BranchRestore}{\text{\textbf{branchRestore}}}
\newcommand{\BTrackRestore}{\text{\textbf{backtrackRestore}}}
\newcommand{\updateStack}{\text{\textbf{updateStack}}}
\newcommand{\SafeResource}{\code{S}.\code{R}} 
\newcommand{\SafeBNResource}{\code{SB}.\code{NR}}
\newcommand{\SafeNNResource}{\code{SNB}.\code{NR}}  
\newcommand{\pop}{\code{pop}}
\newcommand{\UnsafeResource}{\code{U}.\code{R}} 
\newcommand{\UnsafeNResource}{\code{U}.\code{NR}} 
\newcommand{\PBISequent}{\ensuremath{D_{\text{\PBI}}}} 
\newcommand{\LSequent}{\code{LSequent}} 
\newcommand{\HSequent}{\code{HSequent}}
\newcommand{\BIsub}{\code{BI}$_{\code{sub}}$} 
%\newcommand{\BIsub}{\textbf{BI}$_{\textbf{sub}}$} 
\newcommand{\GOI}{\code{G1i}}
\newcommand{\GTI}{\code{G3i}}
\newcommand{\GFI}{\code{G4i}}   
\newcommand{\CMILL}{\code{CMILL}}
\newcommand{\twodagger}{\dagger\!\dagger}
\newcommand{\LJT}{\code{LJT}}
\newcommand{\LabelTest}{\textbf{label\_test} }
\newcommand{\AssignLabel}{\textbf{assign\_label} }
\newcommand{\BBI}{\code{BBI}}
\newcommand{\BI}{\code{BI}}
\newcommand{\LBI}{\code{LBI}}
\newcommand{\LBIT}{\code{LBI2}}
\newcommand{\LBITH}{\code{LBI3}}
\newcommand{\LBITsub}{\text{\code{LBI2}$_{\code{sub}}$}}
\newcommand{\TBI}{\code{TBI}}
\newcommand{\PBI}{\code{PBI}}
\newcommand{\DLBI}{\code{DL}$_{\code{BI}}$}
\newcommand{\dMBI}{\code{dMBI}}
\newcommand{\CBI}{\code{CBI}} 
\newcommand{\LBIsub}{\text{\code{LBI}$_{\code{sub}}$}} 
\newcommand{\phasedepth}{\code{phase\_depth}} 
\newcommand{\sequentweight}{\code{s\_weight}} 
\newcommand{\formulaweight}{\code{f\_weight}}
\newcommand{\sm}[1]{\mbox{\begin{small}$#1$\end{small}}} 
\newcommand{\normalise}{\code{normalise}}
%\newcommand{\BBI}{\textbf{BBI}}
%\newcommand{\BI}{\textbf{BI}}
%\newcommand{\LBI}{\textbf{LBI}}
%\newcommand{\LBIT}{\textbf{LBI2}}
%\newcommand{\LBITsub}{\textbf{LBI2}$_{\textbf{sub}}$}
%\newcommand{\TBI}{\textbf{TBI}}
%\newcommand{\PBI}{\textbf{PBI}}
%\newcommand{\DLBI}{\textbf{DL}$_{\textbf{BI}}$}
%\newcommand{\dMBI}{\textbf{dMBI}}
%\newcommand{\CBI}{\textbf{CBI}} 
%\newcommand{\LBIsub}{\textbf{LBI}$_{\textbf{sub}}$} 
% 
\newcommand{\wand}{$-\!\!*$} 
\newcommand{\CEntry}{\ensuremath{\code{CEntry}\!\!\uparrow}}
\newcommand{\CMultiEntry}{\ensuremath{\code{CMultiEntry}\!\!\uparrow}}
\newcommand{\CbotEntry}{\ensuremath{\code{C}\bot \code{Entry}\!\!\uparrow}}
\newcommand{\CExit}{\ensuremath{\code{CExit}\!\!\downarrow}}
\newcommand{\CbotLock}{\ensuremath{\code{C}{\bot}\code{Lock}\!\!\downarrow}}
\newcommand{\CLock}{\ensuremath{\code{CLock}\!\!\downarrow}}
\newcommand{\BunchesToLock}{\code{BunchesToLock}}
\newcommand{\NRCready}{\text{\em ready-for-clean-\code{\NR}}} 
\newcommand{\NRIready}{\text{\em ready-for-immature-\code{\NR}}}   
\newcommand{\concat}{\text{\textbf{concat}}} 
\newcommand{\stacktop}{\text{\textbf{stackTop}}}
\newcommand{\pickBunch}{\text{\textbf{pickBunch}}}
\newcommand{\record}{\text{\textbf{record}}} 
\newcommand{\HCKn}{\text{\code{HCK}-\code{n}}} 
\newcommand{\HCK}{\text{\code{HCK}}} 
\newcommand{\CKn}{\text{\code{CKn}}}
\newcommand{\Rready}{\text{\em ready-for-\code{\R}}} 
\newcommand{\GenLockScenario}{\text{\textbf{genLockScenario}}} 
\newtheorem{Note}{Note}
%\newtheorem{observation}{Observation} 
%\newtheorem{property}{Property} 
%\newtheorem{myproposal}{Proposed Theorem}
%\newtheorem{algorithm}{Algorithm} 
%\newtheorem{myAxiom}{Axiom}
%\newtheorem{example}{Example}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
%\newtheorem{corollary}{Corollary} 
%\input{notation.tex}
\newcommand{\paper}[1]{ }
\newcommand{\report}[1]{#1}     
%relevant rules.  
\newcommand{\transferUp}{\ensuremath{\code{Transfer}\!\!\uparrow}}
\newcommand{\transferDown}{\ensuremath{\code{Transfer}\!\!\downarrow}}
\newcommand{\relMup}{ 
\AxiomC{$\Omega( ) \vdash_{\psi a} $} 
\RightLabel{$\transferUp$} 
\UnaryInfC{$\Omega \vdash_{\psi} $} 
\DisplayProof
} 
\newcommand{\relMdown}{ 
\AxiomC{$\Omega \vdash_{\psi} $} 
\RightLabel{$\transferDown$} 
\UnaryInfC{$\Omega( ) \vdash_{\psi a} $} 
\DisplayProof
} 
\newcommand{\relUID}{ 
\AxiomC{$\Omega(\Gamma; \bot) \vdash_{\psi} $}  
\RightLabel{$id$} 
\UnaryInfC{$\Omega(\Gamma; a; a^c) \vdash_{\psi}$} 
\DisplayProof 
}  
\newcommand{\relUwedge}{ 
\AxiomC{$\Omega(\Gamma; F_1; F_2) \vdash_{\psi} $} 
\RightLabel{$\wedge$} 
\UnaryInfC{$\Omega(\Gamma; F_1 \wedge F_2) \vdash_{\psi} $} 
\DisplayProof 
} 
\newcommand{\relUvee}{ 
\AxiomC{$\Omega(\Gamma; F_1) \vdash_{\psi} $}  
\AxiomC{$\Omega(\Gamma; F_2) \vdash_{\psi} $} 
\RightLabel{$\vee $}  
\BinaryInfC{$\Omega(\Gamma; F_1 \vee F_2) \vdash_{\psi} $} 
\DisplayProof  
} 
\newcommand{\relUnegTop}{ 
\AxiomC{$\Omega(\Gamma; \bot) \vdash_{\psi}$} 
\RightLabel{$\neg_{\top}$} 
\UnaryInfC{$\Omega(\Gamma; \neg \top) \vdash_{\psi}$} 
\DisplayProof 
} 
\newcommand{\relUnegBot}{ 
\AxiomC{$\Omega(\Gamma;\top) \vdash_{\psi}$} 
\RightLabel{$\neg_{\bot}$} 
\UnaryInfC{$\Omega(\Gamma; \neg \bot) \vdash_{\psi}$} 
\DisplayProof 
} 
\newcommand{\relUnegWedge}{ 
\AxiomC{$\Omega(\Gamma; \neg F_1) \vdash_{\psi}$} 
\AxiomC{$\Omega(\Gamma; \neg F_2) \vdash_{\psi}$} 
\RightLabel{$\neg_{\wedge}$} 
\BinaryInfC{$\Omega(\Gamma; \neg (F_1 \wedge F_2)) \vdash_{\psi}$} 
\DisplayProof 
} 
\newcommand{\relUnegVee}{ 
\AxiomC{$\Omega(\Gamma; \neg F_1; \neg F_2) \vdash_{\psi}$} 
\RightLabel{$\neg_{\vee}$} 
\UnaryInfC{$\Omega(\Gamma; \neg (F_1 \vee F_2)) \vdash_{\psi}$} 
\DisplayProof 
} 
\newcommand{\relUnegNeg}{ 
\AxiomC{$\Omega(\Gamma; a) \vdash_{\psi}$} 
\RightLabel{$\neg_{\neg}$} 
\UnaryInfC{$\Omega(\Gamma; \neg \neg a) \vdash_{\psi}$} 
\DisplayProof  
} 
\newcommand{\relUnegCircle}{  
\AxiomC{$\Omega(\Gamma; a) \vdash_{\psi}$} 
}
%cl+m1/il+m2 
\newcommand{\cimAxO}{ 
\AxiomC{}
\RightLabel{$Ax_1$} 
\UnaryInfC{$\Gamma; a; \neg a \vdash_1$}  
\DisplayProof
}
\newcommand{\cimTopR}{
\AxiomC{}
\RightLabel{$\top R_1$} 
\UnaryInfC{$\Gamma \vdash_1 \Psi_1(\top; \Delta)$} 
\DisplayProof 
}   
\newcommand{\ccollapse}{\ensuremath{\code{PCollapse}\!\uparrow}} 
\newcommand{\inv}{\code{inv}}
\newcommand{\cimCCollapse}{ 
\AxiomC{$D^p \quad (D^p = \observe(D))$} 
\RightLabel{$\ccollapse$} 
\UnaryInfC{$D$}
\DisplayProof
} 
\newcommand{\cimWedgeL}{ 
\AxiomC{$\Gamma; F; G \vdash_1$} 
\RightLabel{$\wedge L_1$} 
\UnaryInfC{$\Gamma; F \wedge G \vdash_1$} 
\DisplayProof
}  
\newcommand{\cimWedgeR}{ 
\AxiomC{$\Gamma_1 \vdash_1 \Psi_1(\Delta; F)$} 
\AxiomC{$\Gamma_1 \vdash_1 \Psi_1(\Delta; G)$} 
\RightLabel{$\wedge R_1$} 
\BinaryInfC{$\Gamma_1 \vdash_1 \Psi_1(\Delta; F \wedge G)$} 
\DisplayProof 
} 
\newcommand{\cimVeeL}{
\AxiomC{$\Gamma; F \vdash_1$} 
\AxiomC{$\Gamma; G \vdash_1$} 
\RightLabel{$\vee L_1$} 
\BinaryInfC{$\Gamma; F \vee G \vdash_1$} 
\DisplayProof
} 
\newcommand{\cimVeeR}{ 
\AxiomC{$\Omega_1 \vdash_1 \Psi_1(\Delta; F; G)$} 
\RightLabel{$\vee R_1$} 
\UnaryInfC{$\Omega_1 \vdash_1 \Psi_1(\Delta; F \vee G)$} 
\DisplayProof
}   
\newcommand{\cimSimLbot}{ 
\AxiomC{$\Gamma; \bot \vdash_1$} 
\RightLabel{$\neg L_{\bot}$} 
\UnaryInfC{$\Gamma; \neg \top \vdash_1$} 
\DisplayProof 
}  
\newcommand{\cimSimLtop}{ 
\AxiomC{$\Gamma \vdash_1$} 
\RightLabel{$\neg L_{\top}$} 
\UnaryInfC{$\Gamma; \neg \bot \vdash_1$} 
\DisplayProof 
}  
\newcommand{\cimSimLwedge}{ 
\AxiomC{$\Gamma; \neg F_1 \vdash_1$}  
\AxiomC{$\Gamma; \neg F_2 \vdash_1$} 
\RightLabel{$\neg L_{\wedge}$} 
\BinaryInfC{$\Gamma; \neg (F_1 \wedge F_2) \vdash_1$} 
\DisplayProof
} 
\newcommand{\cimSimLvee}{ 
\AxiomC{$\Gamma; \neg F_1; \neg F_2 \vdash_1$} 
\RightLabel{$\neg L_{\vee}$} 
\UnaryInfC{$\Gamma; \neg (F_1 \vee F_2) \vdash_1$} 
\DisplayProof 
} 
\newcommand{\cimSimLrightarrow}{  
\AxiomC{}
\RightLabel{$\neg L_{\supset_1}$} 
\UnaryInfC{$\Gamma; \neg (F \supset G) \vdash_1$} 
\DisplayProof
} 
\newcommand{\cimTrightarrowLrightarrow}{ 
\Axiom{$\Omega(\Gamma; F_2 \supset F_3) \vdash F_1^{\uparrow} 
\supset F_2$} 
}
\newcommand{\cimSimR}{ 
\AxiomC{$\Omega_1(\Gamma; F) \vdash_1 \Psi_1(\Delta)$} 
\RightLabel{$\sim R_1$} 
\UnaryInfC{$\Omega_1(\Gamma) \vdash_1 \Psi_1(\Delta; \sim F)$} 
\DisplayProof 
} 
\newcommand{\cimWkL}{ 
\AxiomC{$\Gamma \vdash_1 \Delta$} 
\RightLabel{$Wk L_1$} 
\UnaryInfC{$\Gamma; F \vdash_1 \Delta$} 
\DisplayProof
}   
\newcommand{\cimWkR}{ 
\AxiomC{$\Gamma \vdash_1 \Delta$} 
\RightLabel{$Wk R_1$} 
\UnaryInfC{$\Gamma \vdash_1 \Delta; F$} 
\DisplayProof 
} 
\newcommand{\cimCtrL}{ 
\AxiomC{$\Gamma; F; F \vdash_1 \Delta$} 
\RightLabel{$Ctr L_1$} 
\UnaryInfC{$\Gamma; F \vdash_1 \Delta$} 
\DisplayProof
}  
\newcommand{\cimCtrR}{ 
\AxiomC{$\Gamma \vdash_1 \Delta; F; F$} 
\RightLabel{$Ctr R_1$} 
\UnaryInfC{$\Gamma \vdash_1 \Delta; F$} 
\DisplayProof
} 
\newcommand{\cimBoxL}{  
\AxiomC{$\Gamma; \Box F \vdash_1 \Delta$} 
\RightLabel{$\Box L_1$}   
\UnaryInfC{$ownw \vdash_1 on$} 
\DisplayProof 
} 
\newcommand{\cimBoxR}{ 
\AxiomC{$\Gamma \vdash_1 \Delta; \Box_c F$} 
\RightLabel{$\Box R_1$} 
\UnaryInfC{$\Gamma \vdash_1 \Delta; \Box_c F$} 
\DisplayProof
}  
\newcommand{\cimDiamondL}{ 
\AxiomC{$\Gamma; \Diamond_c F \vdash_1 \Delta$} 
\RightLabel{$\Diamond L_1$} 
\UnaryInfC{$\Gamma \vdash_1 \Delta; \Diamond_c F$} 
\DisplayProof
} 
%%%%cl+m1/il+m2, il+m2
\newcommand{\cimTax}{ 
\AxiomC{}
\RightLabel{$Ax_2$} 
\UnaryInfC{$\Gamma; a \vdash_2 a$}   
\DisplayProof 
}   
\newcommand{\cimSimLsim}{ 
\AxiomC{$\Gamma; F \vdash_1$} 
\RightLabel{$\neg L_{\neg}$} 
\UnaryInfC{$\Gamma; \neg \neg F \vdash_1$} 
\DisplayProof
}
\newcommand{\cimBotL}{ 
\AxiomC{}
\RightLabel{$\bot L_1$} 
\UnaryInfC{$\Gamma; \bot \vdash_1$} 
\DisplayProof
} 
\newcommand{\cimTbotL}{ 
\AxiomC{}
\RightLabel{$\bot L_2$} 
\UnaryInfC{$\Gamma; \bot \vdash_2 H$} 
\DisplayProof 
} 
\newcommand{\cimTtopR}{ 
\AxiomC{}
\RightLabel{$\top R_2$} 
\UnaryInfC{$\Gamma \vdash_2 \top$} 
\DisplayProof 
}  
\newcommand{\cimTwedgeL}{ 
\AxiomC{$\Omega_2(\Gamma; F; G) \vdash_2 H$} 
\RightLabel{$\wedge L_2$} 
\UnaryInfC{$\Omega_2(\Gamma; F \wedge G) \vdash_2 H$} 
\DisplayProof
} 
\newcommand{\cimTwedgeR}{ 
\AxiomC{$\Omega_2 \vdash_2 H_1$} 
\AxiomC{$\Omega_2 \vdash_2 H_2$} 
\RightLabel{$\wedge R_2$} 
\BinaryInfC{$\Omega_2 \vdash_2 H_1 \wedge H_2$} 
\DisplayProof 
} 
\newcommand{\cimTveeL}{ 
\AxiomC{$\Omega_2(\Gamma; F) \vdash_2 H$} 
\AxiomC{$\Omega_2(\Gamma; G) \vdash_2 H$} 
\RightLabel{$\vee L_2$} 
\BinaryInfC{$\Omega_2(\Gamma; F \vee G) \vdash_2 H$} 
\DisplayProof 
} 
\newcommand{\cimTveeR}{ 
\AxiomC{$\Omega_2 \vdash_2 H_i$} 
\RightLabel{$\vee R_2$} 
\UnaryInfC{$\Omega_2 \vdash_2 H_1 \vee H_2$} 
\DisplayProof 
}  
\newcommand{\cimTrightarrowL}{  
\AxiomC{$\Gamma; F \supset G \vdash_2 F$}   
\AxiomC{$\Gamma; G \vdash_2 H$} 
\RightLabel{$\supset L_2$} 
\BinaryInfC{$\Gamma; F \supset G \vdash_2 H$} 
\DisplayProof 
} 
\newcommand{\cimTrightarrowRwedge}{ 
\AxiomC{$\Gamma \vdash H_1^{\uparrow} \supset 
(H_2 \supset H_3); \Delta$}  
\RightLabel{$\supset R_{\wedge}$}  
\UnaryInfC{$\Gamma \vdash (H_1^{\uparrow} \wedge 
H_2) \supset H_3; \Delta$}  
\DisplayProof
}
\newcommand{\cimTrightarrowRc}{ 
\AxiomC{$[\Gamma]; H_1^p \vdash H_2; H_1^p \supset H_2$}  
\RightLabel{$\supset R_c$} 
\UnaryInfC{$\Gamma \vdash H_1^p \supset H_2; \Delta$} 
\DisplayProof 
}  
\newcommand{\cimTrightarrowRi}{ 
\AxiomC{$[\Gamma]; H_1^{\uparrow} \vdash \persist(H_2)$} 
\RightLabel{$\supset R_i$} 
\UnaryInfC{$\Gamma \vdash H_1^{\uparrow} \supset H_2; \Delta$} 
\DisplayProof 
} 
\newcommand{\cimTrightarrowR}{ 
\AxiomC{$\Gamma; H_1 \vdash_2 H_2$}  
\RightLabel{$\supset R_2$} 
\UnaryInfC{$\Gamma \vdash_2 H_1 \supset H_2$} 
\DisplayProof 
}   
\newcommand{\liftUp}{\ensuremath{\code{Lift}\!\uparrow}} 
\newcommand{\cimMwedgeL}{ 
\AxiomC{$\Gamma; F; G \vdash \Delta$} 
\RightLabel{$\wedge L$} 
\UnaryInfC{$\Gamma; F \wedge G \vdash \Delta$} 
\DisplayProof 
} 
\newcommand{\cimMrightarrowLrightarrow}{  
\AxiomC{$[\Gamma; F_2 \supset F_3] \vdash F_1 \supset F_2; 
[\Delta]$}  
\AxiomC{$\Gamma; F_3 \vdash [\Delta]$}  
\RightLabel{$\supset L_{\supset}$} 
\BinaryInfC{$\Gamma; (F_1 \supset F_2) \supset F_3 \vdash 
\Delta$}  
\DisplayProof 
}   
\newcommand{\cimMrightarrowLrightarrowI}{ 
\AxiomC{$[\Gamma; p; F] \vdash [\Delta]$}  
\RightLabel{$\supset L_{p}$} 
\UnaryInfC{$\Gamma; p; p \supset F \vdash \Delta$} 
\DisplayProof 
}
\newcommand{\cimMrightarrowLSim}{  
\AxiomC{$[\Gamma; F_1^{c} \supset F_2] \vdash F_1^{c}; [\Delta]$} 
\AxiomC{$[\Gamma; F_2] \vdash [\Delta]$} 
\RightLabel{$\supset L_{c}$} 
\BinaryInfC{$\Gamma; F_1^c \supset F_2 \vdash \Delta$} 
\DisplayProof 
} 
\newcommand{\cimMveeL}{ 
\AxiomC{$\Gamma; F \vdash \Delta$} 
\AxiomC{$\Gamma; G \vdash \Delta$} 
\RightLabel{$\vee L$} 
\BinaryInfC{$\Gamma; F \vee G \vdash \Delta$} 
\DisplayProof 
}   
\newcommand{\cimMwedgeR}{ 
\AxiomC{$\Gamma \vdash \Delta; H_1$} 
\AxiomC{$\Gamma \vdash \Delta; H_2$} 
\RightLabel{$\wedge R$} 
\BinaryInfC{$\Gamma \vdash \Delta; H_1 \wedge H_2$} 
\DisplayProof 
}  
\newcommand{\cimMveeR}{ 
\AxiomC{$\Gamma \vdash \Delta; H_1; H_2$} 
\RightLabel{$\vee R$} 
\UnaryInfC{$\Gamma \vdash \Delta; H_1 \vee H_2$} 
\DisplayProof 
}  
\newcommand{\cimMrightarrowLvee}{ 
\AxiomC{$\Gamma; F_1 \supset G; F_2 \supset G \vdash 
\Delta$} 
\RightLabel{$\supset L_{\vee}$} 
\UnaryInfC{$\Gamma; (F_1 \vee F_2) \supset G \vdash 
\Delta$} 
\DisplayProof 
} 
\newcommand{\cimMrightarrowLwedge}{ 
\AxiomC{$\Gamma; F_1^{\uparrow} \supset (F_2 \supset F_3) \vdash 
\Delta$} 
\RightLabel{$\supset L_{\wedge}$} 
\UnaryInfC{$\Gamma; (F_1^{\uparrow} \wedge F_2 
\supset F_3) 
\vdash \Delta$} 
\DisplayProof 
}
\newcommand{\cimMrightarrowL}{ 
\AxiomC{$\Gamma; F \supset G \vdash F$} 
\AxiomC{$\Gamma; G \vdash H$}  
\RightLabel{$\supset L$} 
\BinaryInfC{$\Gamma; F \supset G \vdash H$} 
\DisplayProof  
} 
\newcommand{\cimMsimL}{ 
\AxiomC{$\Gamma; F \vdash H$} 
\RightLabel{$\sim L$} 
\UnaryInfC{$\Gamma; \sim \sim F \vdash H$} 
\DisplayProof 
} 
\newcommand{\cimUp}{
\AxiomC{$D \quad [D = \code{lift}(D^I)]$}  
\RightLabel{$\liftUp$} 
\UnaryInfC{$D^I$} 
\DisplayProof
} 
\newcommand{\cimDown}{ 
\AxiomC{$D^I \quad [D^I = \proj_I(D)]$} 
\RightLabel{$\icollapse$} 
\UnaryInfC{$D$} 
\DisplayProof
} 
%%%%%%%%%%%e cl+m1/il+m2
\newcommand{\ax}{ 
\AxiomC{}
\RightLabel{Ax} 
\UnaryInfC{$\Omega_1(p) \vdash_1 p$} 
\DisplayProof
}  
\newcommand{\unitR}{ 
\AxiomC{}  
\RightLabel{{\mtop} R} 
\UnaryInfC{${\mtop} \vdash_1 {\mtop}$}  
\DisplayProof
}
\newcommand{\starL}{ 
\AxiomC{$\Omega_1(\Gamma, F, G) \vdash_1 H$} 
\RightLabel{$* L$} 
\UnaryInfC{$\Omega_1(\Gamma, F * G) \vdash_1 H$} 
\DisplayProof
} 
\newcommand{\starR}{ 
\AxiomC{$\Gamma_1 \vdash_1 H_1$} 
\AxiomC{$\Gamma_2 \vdash_1 H_2$}  
\RightLabel{$* R$} 
\BinaryInfC{$\Gamma_1, \Gamma_2 \vdash_1 H_1 * H_2$} 
\DisplayProof
} 
\newcommand{\stararrowL}{ 
\AxiomC{$\Gamma_1 \vdash_1 F$} 
\AxiomC{$\Omega_1(\Gamma_2, G) \vdash_1 H$} 
\RightLabel{${\text{\lollipop}} L$} 
\BinaryInfC{$\Omega_1(\Gamma_1, \Gamma_2, F {\text{\lollipop}} G) \vdash_1
H$} 
\DisplayProof
} 
\newcommand{\stararrowR}{ 
\AxiomC{$\Gamma_1, F \vdash_1 G$} 
\RightLabel{${\text{\lollipop}} R$} 
\UnaryInfC{$\Omega_1 \vdash_1 F {\text{\lollipop}} G$}  
\DisplayProof
} 
\newcommand{\AX}{ 
\AxiomC{}
\RightLabel{$Ax2$} 
\UnaryInfC{$\Omega_2(\Gamma; p) \vdash_2 p$} 
\DisplayProof
} 
\newcommand{\topR}{ 
\AxiomC{}
\RightLabel{$\top R$} 
\UnaryInfC{$\Omega_2 \vdash_2 \top$} 
\DisplayProof
} 
\newcommand{\botL}{ 
\AxiomC{}
\RightLabel{$\bot L$} 
\UnaryInfC{$\Omega_2(\bot) \vdash_2 \Delta$} 
\DisplayProof 
} 
\newcommand{\wedgeL}{
\AxiomC{$\Omega_2(\Gamma; F; G) \vdash_2 \Delta$} 
\RightLabel{$\wedge L$} 
\UnaryInfC{$\Omega_2(\Gamma; F \wedge G) \vdash_2 \Delta$} 
\DisplayProof
} 
\newcommand{\veeL}{ 
\AxiomC{$\Omega_2(\Gamma; F) \vdash_2 \Delta$} 
\AxiomC{$\Omega_2(\Gamma; G) \vdash_2 \Delta$} 
\RightLabel{$\vee L$} 
\BinaryInfC{$\Omega_2(\Gamma; F \vee G ) \vdash_2 \Delta$}
\DisplayProof
} 
\newcommand{\wedgeR}{ 
\AxiomC{$\Omega_2 \vdash_2 \Delta; F$} 
\AxiomC{$\Omega_2 \vdash_2 \Delta; G$} 
\RightLabel{$\wedge R$} 
\BinaryInfC{$\Omega_2 \vdash_2 \Delta; F \wedge G$} 
\DisplayProof
} 
\newcommand{\veeR}{ 
\AxiomC{$\Omega_2 \vdash_2 \Delta; F; G$} 
\RightLabel{$\vee R$} 
\UnaryInfC{$\Omega_2 \vdash_2 \Delta; F \vee G$} 
\DisplayProof
} 


\endinput

